PROMPT2BOX:Improving LLM Weakness Discovery and Specificity Estimation by Uncovering Entailment Structure among Prompts

To discover the weaknesses of LLMs, researchers often embed prompts into a vector space and cluster them to extract insightful patterns. However, vector embeddings primarily capture topical similarity; as a result, prompts that share a topic but differ in specificity, and consequently in difficulty, are often represented similarly, making fine-grained weakness analysis difficult. To address this limitation, we propose Prompt2Box, which embeds prompts into a box embedding space using a trained encoder. The encoder, trained on existing and synthesized datasets, outputs box embeddings that capture not only semantic similarity but also specificity relations between prompts (e.g., "writing an adventure story" is more specific than "writing a story"). We further develop a novel dimension reduction technique for box embeddings to facilitate dataset visualization and comparison. Our experiments demonstrate that box embeddings consistently capture prompt specificity better than vector baselines and achieve 45% error reduction on average in predicting specificity compared to the prompt length baseline. On the downstream task of creating hierarchical clustering trees for 17 LLMs from the UltraFeedback dataset, Prompt2Box can identify 13.5% more LLM weaknesses than vector baselines and achieves an approximately 33% stronger correlation between hierarchical depth and instruction specificity. The code is available at https://github.com/zawedcvg/box_embeddings.

==> contents/evaluation.tex <==
\section{Results}
\label{sec:eval}

\subsection{Intrinsic Metrics}
STS-B

We can see from \ref{combined_stsb_plot} that while vector does perform better than box, it does so by a margin of about 6\%. Further we see that score of box on just similarity is about 76\%, but after training it with the entailment data, we see the score drop to 66\%. Adding the links, despite it being only around 2000 samples brings the score back to 76\%.

\subsubsection{Top-k results}

Table~\ref{tab:rmse-icml} shows that based on the score difference or whatever, we get better results?(i am thinking of not having separate sections. conclusions too short?)

\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Vec} & \textbf{Box} & \textbf{Rand} \\
\midrule
LLaMA2-13B & 1.482 & \textbf{1.453} & 1.763 \\
Alpaca-7B & 1.788 & \textbf{1.685} & 2.039 \\
Vicuna-33B & 1.593 & \textbf{1.525} & 1.863 \\
\bottomrule
\end{tabular}
\caption{RMSE (lower is better). Average when taken with 6 random neighbors}
\label{tab:rmse-icml}
\end{table}

Followbench results

Box with the entailment training does significantly better than vector in this particular measure. Indicating that it is capturing both relevance and entailmetn stuff..
        
\begin{table}[h]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Method} & \textbf{Value} \\
\hline
vector & 0.64 \\
box with entailment & 0.737 \\
box without entailment & 0.6915  \\
random & 0.503 \\
\hline
\end{tabular}
\caption{Your caption here}
\label{tab:results}
\end{table}
Volume-Length Correlations

We also do a for volume and length. In general, longer prompts will tend to contain more constraints. So we measure. We notice high correlation. says something? idk.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{combined_cumulative_line_graphs_min_size_2.pdf}
    \caption{Enter Caption}
    \label{fig:placeholder}
\end{figure}

\subsection{LLM Weakness Finding and Fixing}
Hierarchical clustering

Score difference: 

Score difference on the three models show that score difference are slightly better for ... in most except in alpaca-7b, where see a big improvement in performance \ref{fig:score_diff_hierarchical}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/clustering_method_comparison.pdf}
    \caption{result with score difference}
    \label{fig:score_diff_hierarchical}
\end{figure}

For the first results we show that it the score difference with neighboring is lower. good... Next is the specificity, while vector is almost the same as random, we see a big increase for box, indicating the ability to capture both semantic and specificity.


        
%Skillverse results going to skip results for this for now.

\subsection{Visualization and Analysis}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{dataset_mix_visualisation.png}
    \caption{Enter Caption}
    \label{fig:placeholder}
\end{figure}


comparing different datasets~\citep{wu2025mapping}

correlation stats for the different dataset visualisation


Volume Correlations:
  Pearson:  0.625671
  Spearman: 0.762397

Similarity Matrix Correlations:
  Pearson:  0.897987
  Spearman: 0.882104

Entailment Matrix Correlations:
  Pearson:  0.762623
  Spearman: 0.825973

